Automated Customized Bug-Benchmark Generation

We introduce Bug-Injector, a system that automatically creates benchmarks for customized evaluation of static analysis tools. We share a benchmark generated using Bug-Injector and illustrate its efficacy by using it to evaluate the recall of two leading open-source static analysis tools: Clang Static Analyzer and Infer. Bug-Injector works by inserting bugs based on bug templates into real-world host programs. It runs tests on the host program to collect dynamic traces, searches the traces for a point where the state satisfies the preconditions for some bug template, then modifies the host program to inject a bug based on that template. Injected bugs are used as test cases in a static analysis tool evaluation benchmark. Every test case is accompanied by a program input that exercises the injected bug. We have identified a broad range of requirements and desiderata for bug benchmarks; our approach generates on-demand test benchmarks that meet these requirements. It also allows us to create customized benchmarks suitable for evaluating tools for a specific use case (e.g., a given codebase and set of bug types). Our experimental evaluation demonstrates the suitability of our generated benchmark for evaluating static bug-detection tools and for comparing the performance of different tools.

==> texfiles/arch-overview.tex <==
\tikzstyle{move} = [->,very thick, color=gt@dkgray]
\tikzstyle{src} = [draw, fill=gt@yellow!30, rounded corners,
  minimum height=4em, text width=5em, text centered]
\tikzstyle{vuln} = [src, fill=gt@blue!30, minimum height=3em, text width=7em]
\tikzstyle{act} = []
\tikzstyle{pop} = [draw, fill=gt@plum!30, circle, text width=6em, text centered]
\tikzstyle{action} = [font=\small\it]

\begin{tikzpicture}[node distance=16ex]
  \node[pop] (pop) {Candidate\\ Population};

  \node[src, fill=gt@blue!30, left=5ex of pop] (host) {Original\\ Program};

  \node[src, fill=gt@red!30, right=5ex of pop] (output) {Vulnerable\\ Program};

  \node[right=14ex of output] (placeholder) {};

  \node[act, below left=14.5ex and 8ex of pop, text width=6em, text centered] (mut) {Mutate \&\\ Instrument};

  \node[act, text centered, right=6ex of mut] (trace)
       {Run};

  \node[act, below right=16ex and 12ex of pop] (eval) {Evaluate};

  \node[act, text centered, left=6ex of eval] (inject)
       {Inject};

  \node[below=3ex of pop,text width=6em, text centered] (evo)
       {Evolutionary\\ Search};
  \draw[move,->,bend right] (evo.40) to (evo.140);
  \draw[move,->,bend right] (evo.220) to (evo.320);

  %% Vulnerabilities
  \node[vuln, below right=2ex and 0ex of inject.south west] (vuln1) {};
  \node[vuln, below right=0.5ex of vuln1.north west] (vuln2) {};
  \node[vuln, below right=0.5ex of vuln2.north west] (vuln3) {};
  \node[vuln, below right=0.5ex of vuln3.north west] (vuln4) {Vulnerabilities};

  %% Inputs
  \node[vuln, below left=2ex and 0ex of trace.south east] (input1) {};
  \node[vuln, below right=0.5ex of input1.north west] (input2) {};
  \node[vuln, below right=0.5ex of input2.north west] (input3) {};
  \node[vuln, below right=0.5ex of input3.north west] (input4) {Inputs};

  %% Mutation Sidebar
  \node[draw, thick, dotted, inner sep=1em, inner xsep=0.5em, text width=15em,
        below left=2ex and 2ex of host.north west]
       (mut-side) {Mutate \& Instrument\\
    \begin{itemize}[noitemsep,nolistsep,leftmargin=*]
    \item Weakening mutation
    \item Camouflage mutation
    \item Instrumentation
    \end{itemize}
    };
  \draw[move,dotted,<->] (mut-side) to (mut);

  %% Widening Sidebar
  \node[draw, thick, dotted, inner sep=1em, text width=13em, below=11ex
    of mut-side]
       (wide-side) {Input generation\\
    \begin{itemize}[noitemsep,nolistsep,leftmargin=*]
    \item Tools
    \item Targeted
    \end{itemize}
    };
  \draw[move,dotted,<->] (wide-side) to (trace.south west);

  %% Evaluation Sidebar
  \node[draw, thick, dotted, inner sep=1em, text width=12em,
        below right=2ex and 2ex of output.north east]
       (eval-side) {Fitness function\\ 
   \begin{itemize}[noitemsep,nolistsep,leftmargin=*]
    \item Camouflage
    \item Distribution
    \item Original functionality
    \end{itemize}
    };
  \draw[move,dotted,<->] (eval-side) to (eval);

  %% Inject Sidebar
  \node[draw, thick, dotted, inner sep=1em, text width=12em, below
    right=0ex and 2ex of output.east, below=8ex of eval-side]
  (inject-side) {Vuln. injection\\
    \hspace*{-3.5ex}
    \begin{tabular}{ccc}
      ~Concrete\hspace{-0.5em} &                   & \hspace{-0.25em}Symbolic     \\
      values\hspace{-0.75em}   & $\Leftrightarrow$ & \hspace{-0.5em}preconditions \\
      ~in Host\hspace{-0.5em}  &                   & \hspace{-0.25em}in Vuln.     \\
  \end{tabular}};
  \draw[move,dotted,<->] (inject-side) to (inject.south east);

  %% Draw
  \draw[move,->] (host) to (pop);
  \draw[move,->] (pop) to (output);

  \draw[move,->,bend right] (pop.205) to node[auto] {Select} (mut);
  \draw[move,->] (mut) to (trace);
  \draw[move,->] (trace) to
    node[auto,above,action] {Trace}
    node[auto,below,action] {Points}
    (inject);
  \draw[move,->] (inject) to (eval);
  \draw[move,->] (input3) to (trace);
  \draw[move,->] (vuln3) to (inject);
  \draw[move,->,bend right] (eval) to node[auto] {Insert} (pop.335);

\end{tikzpicture}

